A Structured Prediction Approach for Missing Value Imputation

Missing value imputation is an important practical problem. There is a large body of work on it, but there does not exist any work that formulates the problem in a structured output setting. Also, most applications have constraints on the imputed data, for example on the distribution associated with each variable. None of the existing imputation methods use these constraints. In this paper we propose a structured output approach for missing value imputation that also incorporates domain constraints. We focus on large margin models, but it is easy to extend the ideas to probabilistic models. We deal with the intractable inference step in learning via a piecewise training technique that is simple, efficient, and effective. Comparison with existing state-of-the-art and baseline imputation methods shows that our method gives significantly improved performance on the Hamming loss measure.

==> ssmv_arxiv/experimental_section.tex <==
%\documentclass[twoside]{article}
%\usepackage{aistats2014,graphics,amsmath,lipsum,multicol,verbatim,array}
%% If your paper is accepted, change the options for the package
%% aistats2014 as follows:
%%
%%\usepackage[accepted]{aistats2014}
%%
%% This option will print headings for the title of your paper and
%% headings for the authors names, plus a copyright note at the end of
%% the first column of the first page.
%
%
%\begin{document}

% If your paper is accepted and the title of your paper is very long,
% the style will print as headings an error message. Use the following
% command to supply a shorter title of your paper so that it can be
% used as headings.
%
%\runningtitle{I use this title instead because the last one was very long}

% If your paper is accepted and the number of authors is large, the
% style will print as headings an error message. Use the following
% command to supply a shorter version of the authors names so that
% they can be used as headings (for example, use only the surnames)
%
%\runningauthor{Surname 1, Surname 2, Surname 3, ...., Surname n}

%\twocolumn[
%
%\aistatstitle{A Large Margin Structured Prediction Learning Approach for Missing Value Imputation}
%
%\aistatsauthor{ Anonymous Author 1 \And Anonymous Author 2 \And Anonymous Author 3}
%
%\aistatsaddress{ Unknown Institution 1 \And Unknown Institution 2 \And Unknown Institution 3} ]


\section{Experiments}

We present our experimental results from two sets of experiments. The goal of the first set of experiments is to provide evidence that the proposed WWFP based piecewise training method is an order of magnitude faster than state of the art methods; we considered a multi-label supervised learning problem for this study. We found this speed-up gain is very important since the overall imputation method (algorithm~\ref{Algorithm}) typically takes $10$-$15$ iterations. The main focus is the second set of experiments where we show that the proposed large margin based imputation method outperforms state of the art imputation methods on several benchmark datasets.

\subsection{Supervised Learning Experiments}
We considered supervised multi-label classification problem, and we used two benchmark datasets: (1) \textsc{Medical} and \textsc{scene}. These datasets are available at~\url{http://mulan.sourceforge.net/datasets.html}. For the \textsc{Medical} dataset, we considered top 10 output variables selected as per the class proportion; outputs with high class imbalance were dropped. We compared our WWFP method with three state of the art large margin structured prediction model learning methods; the first method is dual decomposition based learning (DDL) method~\cite{Kom11}, and the second method~\cite{Luc13},\cite{Rat07} is a primal stochastic sub-gradient (SSG) method. We use test set Hamming loss as the measure for comparing the performance. On the \textsc{Medical} dataset, all the methods (averaged over 2 splits) gave a test error of 9.36\%, and the training time taken by WWFP, DDL and SSG were 54.6, 349.5 and 4662.6 seconds respectively. On the \textsc{Scene} dataset, the test errors obtained were 11.37\%, 10.62\% and 9.89\%, and the training times were 7.74, 147.7, 6073 seconds. These results clearly show that the proposed method achieves significant training time speed-up without significant loss in accuracy.

\subsection{Missing Value Imputation Experiments}
\subsubsection{Experimental Setup}

\noindent{\bf Datasets} We used four categorical datasets from the UCI repository (\url{http://archive.ics.uci.edu/ml/}). Details of these datasets are listed in table \ref{t1}. Note that none of these datasets contain missing values originally. We introduce missing values completely at random such that a certain fraction of each column of the dataset is missing. In our experiment, we consider 3 missing percentages, i.e., we allow 10/30/50\% of the dataset to be missing.
\begin{table}
\centering
%\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|}
\hline
dataset & \# variables & type\\
\hline
flare & $9$ & multinomial\\
\hline
spect & $22$ & binomial\\
\hline
mushroom & $10$ & multinomial\\
\hline
yeast & $14$ & binomial\\
\hline
\end{tabular}
%}
\caption{Details of various datasets used in the missing value imputation experiments}
\label{t1}
\end{table}

\noindent{\bf Measure for Comparison} We use Hamming loss on the imputed values. We get one table at the end of the optimization from our methods, \textsc{Mode} and \textsc{BF}, and we compare this output with the ground truth table to compute the Hamming loss. \textsc{MICE} and \textsc{MM} are sampling based methods; therefore, these methods can generate multiple imputations. We generate 100 samples, and then compute the expected Hamming loss by averaging over the Hamming loss obtained using these 100 tables.

\noindent{\bf Methods for Comparison} We compare our large margin method with four popular methods in the statistics literature. They are:
\begin{enumerate}
\item \textsc{Mode} (MO): Fills up all missing values in a column with the mode of the observed values in the column.
\item \textsc{Mixture Model} (MM): A model in which each mixture component is a product of univariate distributions over each variable. Inference and learning performed using variational Bayes inference\cite{Win05}.
\item \textsc{Mice} (MICE): State of the art imputation algorithm\cite{Buu11}. Involves an iterative procedure of training predictors over each output variable (by minimizing the logistic loss), keeping the other variables as inputs, and sampling the predictor's output distributions over the states of each variable to generate the imputations of the dataset. Note that both parameter learning and imputation is carried out through sampling the posterior distribution over the model weights and states of the variables respectively.
\item \textsc{Backfitting} (BF): A deterministic version of \textsc{Mice}, where instead of the sampling step, we select the optimal parameters obtained from solving the learning (optimization) problem using hinge loss, and the imputed values are obtained by solving the individual inference problem.
\item \textsc{WWFP-WO} Our proposed method without constraints. Note that imputations are done independently for each row by solving (\ref{infpbm}).
\item \textsc{WWFP-WC} Our proposed method with label and pairwise distribution constraints. In this case, joint inference is needed, as explained in Section 3.3.
\end{enumerate}

\noindent{\bf Implementation Details} To set the regularization constant $\lambda$, we perform a cross validation step as follows. Given the missing value data, we build a model for each $\lambda$. Using the model built, for each column, we predict the observed variables in that column using values for the remaining variables picked from the ground truth data. We average the zero-loss computed on each column. Finally, we choose the constant that gives the minimum loss. To make a fair comparison, we used this approach uniformly for all the methods. We are exploring other cross validation approaches for the missing value data scenario. To evaluate the performance, we create six splits of each dataset, and run all the imputation algorithms on all the splits. The results are averaged across the splits of each dataset and presented.  
%One such method is: (1) construct a dataset by making some observed values missing from the input data with missing values, (2) build a model using this dataset for different $\lambda$ values, and (3) evaluate the performance on the observed values that were made missing. 


\begin{table*}
\setlength{\extrarowheight}{6pt}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
dataset & \textsc{MO} & \textsc{MM} & \textsc{MICE} & \textsc{BF} & \textsc{WWFP-WO} & \textsc{WWFP-WC}\\
\hline
FLARE (10\%) & $34.15\pm1.74$ & $29.59\pm0.76$ & $25.48\pm0.9$ & $20.04\pm1.27$ & $20.75\pm2.07$ & {$\bf19.87\pm1.77$}\\
\hline
SPECT (10\%) & $30.23\pm2.95$ & $31.39\pm1.47$ & $23.76\pm1.45$ & $18.76\pm2.01$ & $17.57\pm1.58$ & {$\bf15.29\pm1.7$}\\
\hline
MUSHROOM (10\%) & $45.39\pm0.88$ & $35.5\pm1.69$ & $27.78\pm0.50$ & {$\bf 25.51\pm0.63$} & $30.95\pm0.97$ & $25.54\pm0.52$\\
\hline
YEAST (10\%) & $23.26\pm0.74$ & $23.99\pm1.73$ & $9.62\pm0.83$ & {$\bf 6.59\pm0.82$} & $9.20\pm0.85$ & $7.00\pm1.48$\\
\hline
\hline
FLARE (30\%) & $34.25\pm0.5$ & $32.89\pm1.12$ & $28.51\pm0.29$ & $23.71\pm0.6$ & $24.86\pm1.24$ & {$\bf22.48\pm0.76$}\\
\hline
SPECT (30\%) & $30.38\pm2.0$ & $31.22\pm0.9$ & $25.8\pm0.67$ & $21.98\pm1.09$ & $19.35\pm1.09$ & {$\bf17.77\pm1.01$}\\
\hline
MUSHROOM (30\%) & $45.57\pm0.62$ & $40.62\pm1.93$ & $30.11\pm4.96$ & $28.56\pm0.48$ & $34.25\pm1.01$ & {$\bf28.27\pm0.57$}\\
\hline
YEAST (30\%) & $23.13\pm0.74$ & $27.01\pm0.55$ & $15.33\pm0.42$ & {$\bf 11.54\pm0.8$} & $13.75\pm0.91$ & $11.7\pm0.63$\\
\hline
\hline
FLARE (50\%) & $34.67\pm0.22$ & $39.3\pm0.9$ & $32.24\pm0.53$ & $27.34\pm0.71$ & $28.7\pm1.12$ & {$\bf25.76\pm0.69$}\\
\hline
SPECT (50\%) & $30.93\pm1.01$ & $33.87\pm0.75$ & $28.86\pm0.29$ & $25.11\pm1.12$ & $28.28\pm1.9$ & {$\bf19.25\pm0.62$}\\
\hline
MUSHROOM (50\%) & $45.59\pm0.46$ & $50.36\pm1.68$ & $38.05\pm0.41$  & $33.96\pm0.53$ & $38.80\pm0.54$ & {$\bf32.7\pm0.36$}\\
\hline
YEAST (50\%) & $23.12\pm0.51$ & $31.66\pm0.36$ & $20.91\pm0.124$  & $15.87\pm0.61$ & $17.77\pm0.8$ & {$\bf15.7\pm0.38$}\\
\hline
\end{tabular}
}
\caption{Hamming Loss (\%) for different percentage of missing data indicated in brackets.}
\label{tbl2}
\end{table*}

%\begin{table*}
%\setlength{\extrarowheight}{6pt}
%\centering
%\resizebox{\linewidth}{!}{
%\begin{tabular}{|c|c|c|c|c|c|c|c|}
%\hline
%dataset & \textsc{MO} & \textsc{MM} & \textsc{MICE} & \textsc{BF} & \textsc{WWFP-WO} & \textsc{WWFP-WC}\\
%\hline
%FLARE & $34.25\pm0.5$ & $32.892\pm1.12$ & $28.51\pm0.29$ & $23.71\pm0.6$ & $24.86\pm1.24$ & {$\bf22.48\pm0.76$}\\
%\hline
%SPECT & $30.38\pm2.0$ & $31.22\pm0.9$ & $25.8\pm0.67$ & $21.98\pm1.09$ & $19.35\pm1.09$ & {$\bf17.77\pm1.01$}\\
%\hline
%MUSHROOM & $45.57\pm0.62$ & $40.62\pm1.93$ & $30.11\pm4.96$ & $28.56\pm0.48$ & $34.25\pm1.01$ & {$\bf28.27\pm0.57$}\\
%\hline
%YEAST & $23.13\pm0.74$ & $27.01\pm0.55$ & $15.33\pm0.42$ & {$\bf 11.54\pm0.8$} & $13.75\pm0.91$ & $11.7\pm0.63$\\
%\hline
%\end{tabular}
%}
%\caption{Hamming Loss (\%) with $30$\% missing data}
%%\vspace{-2in}
%\label{tbl3}
%\end{table*}
%\begin{table*}
%\setlength{\extrarowheight}{6pt}
%\centering
%\resizebox{\linewidth}{!}{
%\begin{tabular}{|c|c|c|c|c|c|c|c|}
%\hline
%%dataset & mode & MM & MICE & backfit & LINSVM & LMWO & LMWPC\\
%dataset & \textsc{MO} & \textsc{MM} & \textsc{MICE} & \textsc{BF} & \textsc{WWFP-WO} & \textsc{WWFP-WC}\\
%\hline
%FLARE & $34.67\pm0.22$ & $39.3\pm0.9$ & $32.24\pm0.53$ & $27.34\pm0.71$ & $28.7\pm1.12$ & {$\bf25.76\pm0.69$}\\
%\hline
%SPECT & $30.93\pm1.01$ & $33.87\pm0.75$ & $28.86\pm0.29$ & $25.11\pm1.12$ & $28.28\pm1.9$ & {$\bf19.25\pm0.62$}\\
%\hline
%MUSHROOM & $45.59\pm0.46$ & $50.357\pm1.68$ & $38.05\pm0.41$  & $33.96\pm0.53$ & $38.80\pm0.54$ & {$\bf32.7\pm0.36$}\\
%\hline
%YEAST & $23.12\pm0.51$ & $31.66\pm0.36$ & $20.91\pm0.124$  & $15.87\pm0.61$ & $17.77\pm0.8$ & {$\bf15.7\pm0.38$}\\
%\hline
%\end{tabular}
%}
%\caption{Hamming Loss (\%) with $50$\% missing data}
%%\vspace{-2in}
%\label{tbl4}
%\end{table*}

\subsubsection{Experimental Results}
Experimental results on the benchmark datasets are shown in Tables~{\ref{tbl2}}. The best performance numbers are highlighted in bold. From these tables, the following observations can be made. First, on comparing the last two columns corresponding to our methods without and with constraints clearly demonstrate that significant performance improvement can be achieved by incorporating constraints. Second, the best performance is achieved by \textsc{WWFP-WC} in $9$ out of $12$ cases. In particular, this method starts dominating as the percentage of missingness ($pm$) increases. This is expected because as $pm$ increases, the amount of information available in the data decreases; therefore, additional information such as constraints help in getting improved performance. Similar observation has been made in the semi-supervised learning literature~\cite{Cha13},\cite{Dhi12}.

The performance of \textsc{BF} is close to our method in some cases; and, \textsc{BF} is the second best method. This method has two advantages: (1) it is easy to implement, and (2) is faster compared to our method. When the accuracy performance is of great importance, our method is preferred. The popular \textsc{MICE} method comes next followed by \textsc{MM}. Worst performance was achieved by the simple baseline method \textsc{MO}. This is expected since there is no information used from other variables; also, the estimates are crude.

\section{Discussion and Future Work}

Probabilistic methods such as \textsc{MICE} and \textsc{MM} have the advantage that multiple imputations can be made. This is useful to capture uncertainty in imputations. On doing some detailed analysis, we found that the performance achieved by \textsc{MICE} using the mode computed from the generated samples was found to be good, and very close to \textsc{BF}. However, as the results show, the expected loss is worse; this is because significant mass was present on other samples with high Hamming loss. Similar observation was made with the \textsc{MM} method as well. These observations suggest that there is a need to come out with probabilistic imputation methods that give good performance in expectation. In this context, it is worthwhile to modify our method to make it a probabilistic model. The piecewise learning ideas developed in [3] can be suitably adapted for this purpose.

We observed in our experiments that our method converged in $10$-$15$ iterations. Although we never faced any convergence issue, there is no formal convergence proof to our method. Our method can be improved in the imputation step by changing the optimization problem. For example, instead of solving (\ref{scrimpstep}), we can solve the following optimization problem:
\begin{equation}
\max_{{\bf Y}_m} \sum_{i=1}^n \sum_{q=1}^{Q_i} \sum_{{\bar {\bf u}}_{q,o} \ne {\bf u}^{(i)}_{q,o}} \max(0,\psi^{(i)}({\bar {\bf u}}_{q,o}))^2 \:\: \rm{s.t.}\:\: {\mathcal C}
\label{impstep}
\end{equation}
This formulation has the advantage that the objective function used in the imputation step is also used in the learning step. Therefore, we would expect the objective function to decrease in every step. With bounded objective function value, the method will converge. However, the imputation step becomes complex with the WWFP formulation because of the squared hinge loss term. This term produces higher order potentials in the form of products of scoring functions; for example, multiplying one pairwise scoring function with another results in higher order potentials. Although dual decomposition can be used to solve the problem, the complexity increases and, the overall time taken by the method goes up. On the other hand, higher order potentials would not appear when hinge loss is used; but, the learning step becomes slower due to the non-differentiable nature of the problem. Therefore, there is a trade-off involved in getting overall improvement in speed. This aspect of the problem requires further study.

The proposed method can also be used to solve large margin semi-supervised learning problems for structured outputs. For example, our method can be extended to solve multi-label classification problems, when only partially labeled information is available. The extension is straight-forward as the scoring functions can be appropriately modified to incorporate input features.

While we incorporated distributions based constraints, a detailed study incorporating other types of constraints in different missing value scenarios (e.g., when data is not missing completely at random) is an interesting future work. Finally, though our method can be applied when continuous variables are discretized, coming up with an imputation method that handles mixed data types (e.g., real, categorical and ordinal) directly is another important research problem. 

\section{Conclusion}
We proposed a large margin structured prediction modeling based imputation method to solve the missing value problem. We showed how constraints can be incorporated while imputing the missing values. This is a very powerful feature since consistency checks that are often done to assess the quality of imputation methods can be quantitatively integrated while imputing the missing values. As our experimental results show constraints help in getting significantly improved performance.

%We can think of the constraint as a higher order potential over the entire dataset that is decomposable over each row of the dataset. The label proportion constraint factors into the unary potentials and the correlation constraint factors into the binary potentials.

%Moreover, one of the key contributions of our approach is the incorporation of domain knowledge (encoded as constraints) into the imputation procedure, which is not possible with any of the existing imputation algorithms. Further, we should mention that the framework can incorporate more general constraints, for example, ordinal constraints: if there are two columns such as age and number of years of smoking, it is clear that the second column should always be less than the first. This can be encoded as a label correlation constraint in our setting.
%
%In terms of relative performance of our methods compared to the baselines, we observe the following: Our large margin approach without constraints typically does well in two of the datasets, flare and spect, and is within error bars of the best baselines, particularly with that of backfitting and LINSVM. However, in mushroom and yeast dataset, it does worse than backfitting and LINSVM, although, it does give similar performance compared to Mixture Models and mice.
%
%Our approach with constraints on the other hand, does better than all the competing approaches in almost all the datasets and missing percentages, except mushroom and yeast 10\% setting and yeast 30\% setting. The inclusion of constraints is very important in imputation problems, as many datasets typically are associated with domain knowledge, which when encoded through such constraints, guide the optimization to better solutions, similar to the findings in many semi-supervised learning problems\cite{Cha13}.


%\bibliographystyle{plain}
%\bibliography{PaperBib}
%
%
%\end{document}

